A Survey of Test Time Scaling for Reasoning

Scaling computation at inference time has emerged as a powerful complement to scaling training-time compute, and it drives much of the recent progress in the reasoning abilities of large language models. In this paper, we provide a comprehensive survey of currently popular test-time scaling methods, including parallel sampling, tree search, multi-turn correction, and long chain-of-thought. For each, we examine how it is constructed, how its performance scales with added computation, and how this scaling can be made more efficient. We then compare these methods across multiple dimensions and discuss how they can be effectively combined for enhanced performance. Finally, we discuss how test-time scaling reshapes a broad range of downstream domains, from mathematics and code to multimodal reasoning, agents, and safety, and outline the open challenges and future directions in each.

==> algorithm/iterative_self_reinforced_learning.tex <==
\begin{algorithm}[tb!]
\caption{Iterative Self-reinforced Learning} 
\DontPrintSemicolon
\SetAlgoLined
\KwIn{Original training set $\mathcal{D_\text{0}} = \{x_i, y_i\}$, original query set $\mathcal{D}_\text{0}^{\text{query}} = \{x_i\}$, $M_{\text{0}}$: initial policy model, $T$: iteration times, $R_0$: initial reward model, $\text{Sample}(.)$: policy sample function, $\text{Synthesize}_{\text{query}}(.)$: query synthesis function, $\text{Update}_{\text{policy}}(.)$: policy update function,  $\text{Update}_{\text{reward}}(.)$: reward model update function,  $\text{Filter(.)}$: filter function}
\For{$t = 0$ \KwTo $T-1$}{
     $\mathcal{D}_t^{\text{query}} = \text{Synthesize}_{\text{query}}(\mathcal{D}_{t-1}^{\text{query}}, M_t)$ \;
    $\mathcal{D}_t = \{ (x^i,\{y^i_j\}_{j=1}^{N_i})|_{i=1}^{N_t}$ \text{ s.t. } $x^i \sim \mathcal{D}_t^{query}$, $\{y^i_j\}_{j=1}^{N_i} \sim \text{Sample}(M_t, x^i) \}$ \;
   Annotate $\mathcal{D}_t$ with reward model $R_t$ \;
   $\mathcal{D}_t^{\text{filter}} = \text{Filter}(\mathcal{D}_1, \mathcal{D}_2, ... , \mathcal{D}_t)$ \;
    $M_{t+1} = \text{Update}_{\text{policy}}(M_t, \mathcal{D}_t^{\text{filter}})$ \;
    $R_{t+1} = \text{Update}_{\text{reward}}(R_t, \mathcal{D}_t^{\text{filter}})$
}
\label{alg:iterative_rl}
\end{algorithm}

==> figure/math_comparison.tex <==
\definecolor{lightgreen}{RGB}{220,255,220}

\begin{figure}[tb!]
\centering

\begin{tikzpicture}[
    font=\small, % Set the font size to small
]

% Question box
% Question box
\node[draw, rounded corners=3pt, minimum width=3cm, text width=16cm] (question) {Let $a_0$, $a_1$, $a_2$, $\dots$ be an infinite sequence of real numbers such that $a_0 = \frac{5}{13}$ and $a_{n} = 2a_{n-1}^2 - 1$ for every positive integer $n$. Let $c$ be the smallest number such that for every positive integer $n$, the product of the first $n$ terms satisfies the inequality $|a_0 a_1 \dotsm a_{n - 1}| \le \frac{c}{2^n}$.What is the value of $100c$, rounded to the nearest integer?};

% Answer-only box
\node[draw, rounded corners=3pt, minimum width=1.5cm,  below=0.5cm of question] (answer) {answer: 108};


\node[draw, rounded corners=3pt, minimum width=4.5cm, align=left, text width=16cm, below=0.5cm of answer] (cot) {COT\\
Define the sequence $(\theta_n)$ by $\theta_0 = \arccos \frac{5}{13}$ and $\theta_n = 2 \theta_{n - 1}.$ Then $\cos \theta_0 = \frac{5}{13},$ and $\cos \theta_n &= \cos (2 \theta_{n - 1})= 2 \cos^2 \theta_{n - 1} - 1.$ Since the sequences $(a_n)$ and $(\cos \theta_n)$ have the same initial term, and the same recursion, they coincide. We have that $\sin^2 \theta_0 = 1 - \cos^2 \theta_0 = \frac{144}{169}$. Since $\theta_0$ is acute, $\sin \theta_0 = \frac{12}{13}.$ Now,$ a_0 a_1 \dotsm a_{n - 1} = \cos \theta_0 \cos \theta_1 \dotsm \cos \theta_{n - 1} = \cos \theta_0 \cos 2 \theta_0 \dotsm \cos 2^{n - 1} \theta_0.$ Multiplying both sides by $\sin \theta_0 = \frac{12}{13},$ we get$\frac{12}{13} a_0 a_1 \dotsm a_{n - 1} = \sin \theta_0 \cos \theta_0 \cos 2 \theta_0 \cos 4 \theta_0 \dotsm \cos 2^{n - 1} \theta_0 = \frac{1}{2} \sin 2 \theta_0 \cos 2 \theta_0 \cos 4 \theta_0 \dotsm \cos 2^{n - 1} \theta_0 = \frac{1}{4} \sin 4 \theta_0 \dotsm \cos 2^{n - 1} \theta_0 = \dotsb = \frac{1}{2^n} \sin 2^n \theta_0.$ Hence,$|a_0 a_2 \dotsm a_{n - 1}| = \frac{1}{2^n} \cdot \frac{13}{12} |\sin 2^n \theta_0| \le \frac{1}{2^n} \cdot \frac{13}{12}.$This tells us $c \le \frac{13}{12}.$ We can compute that $a_1 = 2a_0^2 - 1 = 2 \left( \frac{5}{13} \right)^2 - 1 = -\frac{119}{169},$ so $\frac{5}{13} \cdot \frac{119}{169} \le \frac{c}{4}.$ Then $c \ge \frac{2380}{2197}.$  The bound $\frac{2380}{2197} \le c \le \frac{13}{12}$ tells us that the integer closest to $100c$ is $\boxed{108}.$
};

% Long thought box
\node[draw, rounded corners=3pt, minimum width=3cm, align=left, text width=16cm, below=0.5cm of cot]  {Long Thought\\

We have an infinite real number sequence \( a_0, a_1, a_2, \dots \), where the initial term \( a_0 = \frac{5}{13} \).  
The recurrence relation is: $a_n = 2a_{n-1}^2 - 1 \quad \text{for all } n \geq 1$
Our goal is to find the smallest constant $c$ such that for all $n$, the inequality $\left|a_0 a_1 \cdots a_{n-1}\right| \leq \frac{c}{2^n}$
holds true. Ultimately, we need to calculate $100c$ and round it to the nearest integer.


First, we have the recurrence formula: $a_n = 2a_{n-1}^2 - 1$. The initial condition is $a_0 = \frac{5}{13}$.  
To better understand this recurrence relation, we can try calculating the first few terms: $a_1 = 2a_0^2 - 1 = 2\left(\frac{5}{13}\right)^2 - 1 = 2 \times \frac{25}{169} - 1 = \frac{50}{169} - 1 = \frac{50 - 169}{169} = \frac{-119}{169}$. $a_2 = 2a_1^2 - 1 = 2\left(\frac{-119}{169}\right)^2 - 1 = 2 \times \frac{14161}{28561} - 1 = \frac{28322}{28561} - 1 = \frac{28322 - 28561}{28561} = \frac{-239}{28561}$. By calculating the first few terms, we can observe the trend of the sequence $a_n$.  
However, this does not directly help us solve the inequality problem. Therefore, we need to find a more effective method.

The original inequality is: $\left|a_0 a_1 \cdots a_{n-1}\right| \leq \frac{c}{2^n}$. To simplify this inequality, we can multiply both sides by $2^n$: $\left|2a_0 \cdot 2a_1 \cdots 2a_{n-1}\right| \leq c$
This way, we have transformed the inequality into a product form involving $2a_i$. However, while this step simplifies the form of the inequality, it does not immediately reveal how to further handle the product of $2a_i$. Thus, we need to explore other methods to address this recurrence relation.

Observing the recurrence formula: $a_n = 2a_{n-1}^2 - 1$
This resembles the double-angle formula for the cosine function: $\cos(2\theta) = 2\cos^2\theta - 1$
This similarity leads us to the idea that perhaps we can relate the sequence $a_n$ to the cosine function.

Suppose each term $a_n$ can be represented as the cosine of a certain angle. Specifically, let: $a_n = \cos\theta_n$
Thus, the recurrence formula becomes: $\cos\theta_n = 2\cos^2\theta_{n-1} - 1$. According to the double-angle formula, we know: $\cos(2\theta) = 2\cos^2\theta - 1$
Therefore, we can deduce: $\cos\theta_n = \cos(2\theta_{n-1})$. This implies: $\theta_n = 2\theta_{n-1} \quad (\text{or } \theta_n = -2\theta_{n-1} + 2k\pi$, \text{ but here we take the positive angle}). Thus, the relationship between the angles is: $\theta_n = 2\theta_{n-1}$. By iterating further, we obtain: $\theta_n = 2^n \theta_0$
where $\theta_0$ is the initial angle corresponding to $a_0$.

Based on our definition: $a_0 = \cos\theta_0 = \frac{5}{13}$. To find $\theta_0$, we need to calculate: $\theta_0 = \arccos\left(\frac{5}{13}\right)$. Additionally, we can compute: $\sin\theta_0 = \sqrt{1 - \cos^2\theta_0} = \sqrt{1 - \left(\frac{5}{13}\right)^2} = \sqrt{1 - \frac{25}{169}} = \sqrt{\frac{144}{169}} = \frac{12}{13}$
Thus, we have $\sin\theta_0 = \frac{12}{13}$.

Returning to our inequality: $\left|a_0 a_1 \cdots a_{n-1}\right| \leq \frac{c}{2^n}$. Based on our definition $a_i = \cos\theta_i$, we have: $a_0 a_1 \cdots a_{n-1} = \prod_{i=0}^{n-1} \cos\theta_i$. Since $\theta_i = 2^i \theta_0$, we can express the product as: $\prod_{i=0}^{n-1} \cos(2^i \theta_0)$. Using the product formula for cosines, we know: $\prod_{i=0}^{n-1} \cos(2^i \theta_0) = \frac{\sin(2^n \theta_0)}{2^n \sin\theta_0}$. Therefore, the inequality can be transformed to: $\left|\frac{\sin(2^n \theta_0)}{2^n \sin\theta_0}\right| \leq \frac{c}{2^n}$

Multiplying both sides by $2^n \sin\theta_0$ (noting that $\sin\theta_0 > 0$), we obtain: $\left|\sin(2^n \theta_0)\right| \leq c \cdot \sin\theta_0$
Substituting the known $\sin\theta_0 = \frac{12}{13}$, we get: $\left|\sin(2^n \theta_0)\right| \leq c \cdot \frac{12}{13}$. To ensure this inequality holds for all $n$, we require: $c \geq \frac{|\sin(2^n \theta_0)|}{\frac{12}{13}} = \frac{13}{12} |\sin(2^n \theta_0)|$
Since $|\sin(2^n \theta_0)| \leq 1$ for all $n$, the smallest $c$ must satisfy: $c \geq \frac{13}{12}$
Therefore, the smallest $c$ is $\frac{13}{12}$.

The problem requires us to calculate $100c$ and round it to the nearest integer. Based on our value for $c$: $100c = 100 \times \frac{13}{12} = \frac{1300}{12} = 108.\overline{3}$. Rounding $108.\overline{3}$ to the nearest integer, we obtain: $100c \approx 108$
Therefore, the final answer is $108$.
};

\end{tikzpicture}
\caption{Your caption here}
\end{figure}

==> table/supervised_finetuning.tex <==
\begin{table}[tb!]
    \centering
    \scriptsize
\caption{An organization of works on eliciting models' cognitive behaviors through supervised fine-tuning. \textbf{Source} indicates training data origin. \textbf{Quantity} shows training data volume. Under \textbf{Training}, \textbf{Full} denotes full parameter SFT. \textbf{Per.} indicates whether performance is improved. \textbf{Cog.} indicates whether cognitive behaviors are observed after training.}
    \begin{tabular}{l|ccccc|cc}
        \toprule
        \textbf{Work} & \textbf{Application} & \textbf{Source} & \textbf{Quantity} &  \textbf{Training} & \textbf{Model Size} & \textbf{Per.} & \textbf{Cog.} \\
        \midrule
        \rowcolor[rgb]{ .949,  .949,  .949} Searchformer~\cite{lehnert2024abetterplanningtransformers} &  Pathfinding & Synthesize & 50K$\sim$1M  & Full & 15M$\sim$757M & \blackcheck &  \blackcheck \\
        SoS~\cite{gandhi2024streamsearchsoslearning} &  Countdown & Synthesize & 285K & Full & 250M & \blackcheck & \blackcheck  \\       
        \rowcolor[rgb]{ .949,  .949,  .949} O1 Journey–Part 1~\cite{o1journey} & Math & Synthesize & 0.3K & Full & 7B & \blackcheck & - \\
        O1 Journey–Part 2~\cite{o1journeypart2} & Math & Distillation & - & Full & 72B & \blackcheck & \blackcheck \\
        \rowcolor[rgb]{ .949,  .949,  .949} Marco-o1~\cite{zhao2024marcoo1openreasoningmodels} & Translation & Synthesize & 60K & Full  & 7B & \blackcheck & - \\
        STILL-2~\cite{min2024imitateexploreselfimprovereproduction} & Math, Code, Science, Puzzle & Distillation & 5K & Full &  32B & \blackcheck & \blackcheck \\
        \rowcolor[rgb]{ .949,  .949,  .949} AutoMathCritique~\cite{xiEnhancingLLMReasoning2024} & Math & Synthesize & 4K & Full & 8B & \blackcross & - \\
        RedStar~\cite{xu2025redstardoesscalinglongcot} & Math, Code & Distillation & 4K$\sim$1M & Full & 7B$\sim$32B & \blackcheck & \blackcheck  \\
        \rowcolor[rgb]{ .949,  .949,  .949} S1~\cite{muennighoff2025s1simpletesttimescaling} & Math, Science, Code & Distillation & 1K & Full & 32B & \blackcheck & \blackcheck \\
        LIMO~\cite{ye2025limoreasoning} & Math & Distillation & 0.8K & Full & 32B & \blackcheck & \blackcheck \\
        \rowcolor[rgb]{ .949,  .949,  .949} OpenThinker-32B~\cite{openthoughts} & Math, Code, Science, Puzzle & Distillation & 114K & Full & 32B & \blackcheck & \blackcheck \\
        Sky-T1-32B-Preview~\cite{li2025llmseasilylearnreason}  & Math, Code & Distillation & 17K & Full/LoRA & 32B & \blackcheck & \blackcheck \\
        \rowcolor[rgb]{ .949,  .949,  .949} Small-model-gap~\cite{li2025smallmodelsstrugglelearn} & Math & Distillation & 7.5K & Full & 0.5B$\sim$3B & \blackcheck & \blackcheck \\
        Small-model-gap~\cite{li2025smallmodelsstrugglelearn} & Math & Distillation & 7.5K & Full/LoRA & 7B$\sim$32B & \blackcross & \blackcheck \\
        \rowcolor[rgb]{ .949,  .949,  .949} $S^2R$~\cite{ma2025s2rteachingllmsselfverify} & Math & Synthesize & 3K$\sim$4K &Full & 7B  & \blackcheck &\blackcheck \\
        \bottomrule
    \end{tabular}
    \label{tab:sft}
\end{table}
